This Looks Like That... Does it? Shortcomings of Latent Space Prototype Interpretability in Deep Networks

Deep neural networks that yield human interpretable decisions by architectural design have lately become an increasingly popular alternative to post hoc interpretation of traditional black-box models. Among these networks, the arguably most widespread approach is so-called prototype learning, where similarities to learned latent prototypes serve as the basis of classifying an unseen data point. In this work, we point to an important shortcoming of such approaches. Namely, there is a semantic gap between similarity in latent space and similarity in input space, which can corrupt interpretability. We design two experiments that exemplify this issue on the so-called ProtoPNet. Specifically, we find that this network's interpretability mechanism can be led astray by intentionally crafted or even JPEG compression artefacts, which can produce incomprehensible decisions. We argue that practitioners ought to have this shortcoming in mind when deploying prototype-based models in practice.

==> derivation_implications.tex <==
\section{Deriving the Equivalence}
In this section, we motivate our claim that Equivalence~\ref{eq:equivalence} is necessary for a ProtoPNet to be human interpretable.

\citet{chen2018looks} suggest that we can interpret a classification decision by looking at the prototype's which the ProtoPNet found to be most strongly present in the input. For a particular prototype, this means that a user looks at the prototypes visualisation (i.e. a patch of a training image) and the patch in the input image which the ProtoPNet finds most similar to the given prototype. This is indeed similar to how humans communicate their decisions. However, it is only meaningful \emph{if} the other person finds two parts of an object similar for the same reasons. Otherwise, the decision of one person is not understandable to the other. Hence, without such a mutual understanding between a human and a ProtoPNet, displaying prototype similarities does not per-se yield interpretability. Consequently, Equivalence~\ref{eq:equivalence} needs to hold for a ProtoPNet to be interpretable.\\
Indeed, if a human and a ProtoPNet find two image patches similar for different reasons, interpretability would require the human to make sense of the latent representations which are the ProtoPNet's basis for scoring similarity. Yet, these representations are the outputs of a convolutional backbone and can hence not be considered interpretable.


==> remedies.tex <==
\section{Potential Remedies}
We tried one counter-measure per experiment. Specifically, we investigated adversarial training \cite{wong2020fast} to make the optimization problem in the Head-On-Stomach experiment harder. For the JPEG experiment, we simply added JPEG compression to the augmentation pipeline. Both strategies helped to mitigate the problems encountered in the respective experiments. We provide more information and results in Appendix~\ref{app:remadvtraining} and Appendix~\ref{app:remcompression}.
